Comparing Decision Support Approaches for Cyber Security Investment

When investing in cyber security resources, information security managers have to follow effective decision-making strategies. We refer to this as the cyber security investment challenge. In this paper, we consider three possible decision-support methodologies for security managers to tackle this challenge. We consider methods based on game theory, combinatorial optimisation and a hybrid of the two. Our modelling starts by building a framework where we can investigate the effectiveness of a cyber security control regarding the protection of different assets seen as targets in presence of commodity threats. In terms of game theory we consider a 2-person control game between the security manager who has to choose among different implementation levels of a cyber security control, and a commodity attacker who chooses among different targets to attack. The pure game theoretical methodology consists of a large game including all controls and all threats. In the hybrid methodology the game solutions of individual control-games along with their direct costs (e.g. financial) are combined with a knapsack algorithm to derive an optimal investment strategy. The combinatorial optimisation technique consists of a multi-objective multiple choice knapsack based strategy. We compare these approaches on a case study that was built on SANS top critical controls. The main achievements of this work is to highlight the weaknesses and strengths of different investment methodologies for cyber security, the benefit of their interaction, and the impact that indirect costs have on cyber security investment.

==> bibliography.tex <==
\begin{thebibliography}{16}
\bibitem{Deloitte}
Deloitte-NASCIO cyber security Study State governments at risk: a call for collaboration and compliance (2012).
\url{https://www.deloitte.com/assets/Dcom-UnitedStates/Local\%20Assets/Documents/AERS/us_aers_nascio\%20cyber security\%20Study_10192012.pdf}(accessed May 2014).

\bibitem{Manos2014}
Panaousis, E., Fielder, A., Malacaria, P., Hankin, C., Smeraldi, F.: 
Cyber Security Games and Investments: A Decision Support Approach.
In: Proc. of the 5th International Conference on Decision and Game Theory for Security (2014)

\bibitem{Anderson:ACSAC:2001}
Anderson, R:
Why Information Security is Hard. 
In Proc. of the 17th Annual Computer Security Applications Conference (2001)

\bibitem{Kiekintveld:AAMAS:2013}
Kiekintveld, C., Islam, T., Kreinovich, V.: 
Security Games with Interval Uncertainty. 
In: Proc. of the 12th International Conference on Autonomous Agents and Multiagent Systems (AAMAS 2013), pp. 231-238. International Foundation for Autonomous Agents and Multiagent Systems, Richland (2013)

\bibitem{Alpcan:Book:2012}
Alpcan, T., Basar, T.:
Network Security: A Decision and Game-Theoretic Approach. 
Cambridge University Press (2010)

\bibitem{Alpcan:NTMS:2012}
Alpcan, T.: 
Dynamic incentives for risk management.
In: Proc. of the 5th IEEE International Conference on New Technologies, Mobility and Security (NTMS) (2012)

\bibitem{Alpcan:CRiSIS:2009}
Alpcan, T., Bambos, N.:
Modeling dependencies in security risk management. 
In: Proc. of the Fourth International Conference on Risks and Security of Internet and Systems (CRiSIS), pp. 113-116 (2009)

\bibitem{Saad:ICIMP:2010}
Saad, W., Alpcan, T., Basar, T., Hjorungnes, A.: 
Coalitional game theory for security risk management. 
In: Proc. of the 5th International Conference on Internet Monitoring and Protection (ICIMP), pp.\,35-40 (2010)

\bibitem{Bommannavar:ICC:2011}
Bommannavar, P., Alpcan, T., Bambos, N.: 
Security risk management via dynamic games with learning. 
In: Proc. of the 2011 IEEE International Conference on Communications (ICC), pp.\,1-6 (2011)

\bibitem{Fielder:IFIPSEC:2014}
Fielder, A., Panaousis, E., Malacaria, P., Hankin, C., Smeraldi, F.: 
Game theory meets information security management.
In: Proc. of the 29th IFIP International Information Security and Privacy Conference (2014)

\bibitem{Gordon:TISSEC:2002}
Gordon, L.A., Loeb, M.P.: 
The economics of information security investment.
In: ACM Transactions on Information and System Security (TISSEC) (2002)

\bibitem{Johnson:Springer:2012}
Johnson, B., Grossklags, J., Christin, N., Chuang, J.:
Nash equilibria for weakest target security games with heterogeneous agents.
In: Jain, R., Kannan, R. (eds.) Gamenets 2011. LNICST, vol. 75, pp. 444-458. Springer, Heidelberg (2012)

\bibitem{Cavusoglu:JMIS:2014}
Cavusoglu, H., Srinivasan, R., Wei, T.Y.:
Decision-theoretic and game-theoretic approaches to IT security investment.
In: Journal of Management Information Systems(ACySe), 25(2), pp.281-304 (2008)

\bibitem{Smeraldi:ACySe:2014}
Smeraldi, F., Malacaria, P.:
How to Spend it: Optimal Investment for Cyber Security.
In: Proc. of the 1st International Workshop on Agents and cyber security (ACySe) (2014)

\bibitem{Cremonini:WorkingPaper:2006}
Cremonini, M., Nizovtsev, D.:
Understanding and influencing attackers' decisions: Implications for security investment strategies

\bibitem{Dunn2012}
Al-Humaigani, Muhammad, and Derrek B Dunn.: 
A model of return on investment for information systems security. 
argument 4 (2003): 9.

\bibitem{Wang2008}
Wang, Jingguo, Aby Chaudhury, and H. Raghav Rao.: 
Research Note-A Value-at-Risk Approach to Information Security Investment. 
Information Systems Research 19.1 (2008): 106-120.

\bibitem{Demetz:WEIS:2012}
Demetz, L., Bachlechner, D.:
To Invest or Not to Invest? Assessing the Economic Viability of a Policy and Security Configuration Management Tool.
The Economics of Information Security and Privacy, Springer Berlin Heidelberg, pp. 25-47 (2013)

\bibitem{Tsai:2009}
Tsai, J., Kiekintveld, C., Ordonez, F., Tambe, M., Rathi, S.:
IRIS-a tool for strategic security allocation in transportation networks (2009)

\bibitem{minimax}
Von Neumann, J., Morgenstern O.:
Theory of Games and Economic Behavior (60th Anniversary Commemorative Edition). 
Princeton university press (2007)

\bibitem{Nash:NAS:1950}
Nash, J.F.:
Equilibrium points in n-person games. 
In Proc. of the National Academy of Sciences 36(1), pp. 48--49 (1950)

\bibitem{Alpcan:Book:2010}
Alpcan, T., Basar, T.:
Network Security: A Decision and Game-Theoretic Approach. 
Cambridge University Press (2010)

\bibitem{Basar:Book:1995}
Basar, T., Olsder, G. J.:
Dynamic noncooperative game theory.
London Academic press, 2nd Edition (1995)

%\bibitem{SANS:25:2011}
%CWE:
%2011 CWE/SANS Top 25 Most Dangerous Software Errors.
%\url{http://cwe.mitre.org/top25/}
%(accessed May 2014)
%
%\bibitem{CC:20controls:2014}
%Council on cyber security:
%The critical security controls for effective cyber defense (version 5.0).
%\url{http://www.counciloncyber security.org/attachments/article/12/CSC-MASTER-VER50-2-27-2014.pdf}
%(accessed May 2014)
%	
%\bibitem{Deloitte:Report:2012}
%2012 Deloitte-NASCIO cyber security Study State governments at risk: a call for collaboration and compliance.
%\url{https://www.deloitte.com/assets/Dcom-UnitedStates/Local\%20Assets/Documents/AERS/us_aers_nascio\%20cyber security\%20Study_10192012.pdf}
%(accessed May 2014)
